Strike a Chord! Modal Kinetic Typography

We introduce modal kinetic typography, which animates a vector glyph to express a semantic concept while keeping it legible. Our key idea is to build motion from the glyph's natural vibration modes. Specifically, a finite-element eigenproblem assembled from the vector outline yields the glyph's softest modes, for the whole letter and for each of its parts, allowing it to bend. The problem's zero-energy solutions, i.e., rigid translations and rotations, are applied in closed form to each part, allowing parts to also move as blocks. To animate the glyph, a frozen video diffusion model supervises only the modes' amplitudes and phases. Our modal approach addresses two weaknesses of prior work. Free-form point optimization under video score distillation (SDS) moves each point and frame independently along noisy gradients, tearing the outline and causing jitter. In contrast, our modes are smooth along the outline and driven by a few whole-cycle harmonics, which restricts these gradients to smooth, seamlessly looping motion. On the other hand, structured alternatives rely on skeletons or keypoints from category-specific priors, whereas our modes come from the glyph itself; the only prior is a list naming each letter's moving parts, generated once for the whole alphabet by a language model. In modal kinetic typography, shape and motion are disentangled by construction: a single base outline is sculpted toward the concept, and the modal drive cannot alter it, so a letter can also be animated without being reshaped. Our method produces more articulated and smoother motion than Dynamic Typography and AniClipart at comparable or better concept alignment, with less glyph tearing than Dynamic Typography, and is preferred by human raters, including in a frozen-shape setting where motion alone must carry the concept. Our results were also preferred over Astra (GPT-6) by human raters.

==> figs_tex/multi.tex <==
\begin{figure}[!t]
\centering
% Animated in Acrobat / PDF-XChange: the leftmost cell of every strip plays the clip
% while the rest stay static. Other viewers show the poster frame, so the figure still
% reads as a still. Rebuild with: python figs/make_multi_fig.py all
\animategraphics[width=\textwidth,autoplay,loop,poster=first]{8}{figs/multi_anim/frame_}{0}{11}
\caption{\textbf{Two-letter examples.} Three frames per clip. Each letter is its own modal
system with its own concept prompt; the two are rendered together so the prior sees the
pair, and a gradient mask keeps each letter's prompt from reaching the other's parameters.
Identity and orientation hold without leakage. \todoc{placeholder assets from an earlier
model; regenerate under the current configuration.} [gifs better seen in Adobe Acrobat.]}
\label{fig:multi}
\end{figure}


==> figs_tex/work_rel.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=\textwidth]{figs/positioning.pdf}
\caption{
Animation and deformation methods under generative priors, organized by motion structure and semantic guidance.
% \textbf{Where this work sits in vector and animation space:} Related methods placed by how motion is
% structured (horizontal) and what supplies the semantics (vertical). 
% A separate
% line of spectral work does not appear here at all: it analyzes the
% \emph{diffusion process} itself---eigenmodes of the data covariance or of the
% sampler's learning dynamics---rather than of anything that moves. The
% derived-structure, video-SDS corner is empty: methods driven by a video prior
% either optimize point positions freely (Dynamic Typography,
% \citealp{liu2025dynamic}) or depend on authored structure---a skeleton (AKD, Sketch2Motion) or hand-placed
% keypoints (AniClipart, \citealp{wu2025aniclipart}).
% Ours is the only method whose motion basis is derived from the shape itself
% while the semantics come from a video diffusion prior.
}
\label{fig:positioning}
\end{figure}


==> tables/_unused/userstudy_tab.tex <==
\begin{table}[tb]
\centering
\caption{\textbf{User study} results, for the two studies covering our two tasks.}
\label{tab:user}
\small
\begin{tabular}{lccc}
\toprule
Method & Motion $\uparrow$ & Semantics $\uparrow$ & Overall $\uparrow$ \\
\midrule
Dynamic Typography \citep{liu2025dynamic} & $0.89$ & $0.82$ & $0.86$ \\
Astra (Full task)  & $0.79$ & $0.90$ & $0.84$ \\
Ours (Full task)                         & $\mathbf{1.32}$ & $\mathbf{1.28}$ & $\mathbf{1.30}$ \\
\midrule
AniClipart \citep{wu2025aniclipart}        & $1.17$ & -- & $1.17$ \\
Astra (Frozen shape)  & $0.34$ & -- & $0.34$ \\
Ours (Frozen shape)  & $\mathbf{1.48}$ & -- & $\mathbf{1.48}$ \\
\bottomrule
\end{tabular}
\end{table}

==> tables/letterfid_tab.tex <==
\begin{table}[h]
\centering
\caption{\textbf{Letter fidelity, with form weight} in both settings, against Dynamic Typography~\citep{liu2025dynamic}, AniClipart~\citep{wu2025aniclipart} and ASTRA.
The unmarked columns are those of Table~\ref{tab:main}. Dead time is the share of motion
carrying no acceleration, $0$ for a harmonic and $0.75$ for linear interpolation between
keyframes; it is the counterweight to jerk. Reads as letter and form weight ask whether what
moves is still a letter, the latter best at $1$, where the animated form carries the stroke
weight of the glyph it animates. The motion columns repeat Table~\ref{tab:main}; form weight appears only here.}
\label{tab:letterfid}
\footnotesize
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lccccccccc@{}}
\toprule
& \multicolumn{2}{c}{Motion} & \multicolumn{2}{c}{Live motion} & & & & \multicolumn{2}{c}{Letter fidelity} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){9-10}
Method & \shortstack{Global\\$\downarrow$} & \shortstack{Artic.\\$\uparrow$} & \shortstack{Jerk\\$\downarrow$} & \shortstack{Dead\\time $\downarrow$} & \shortstack{Temp.\\cons.\ $\uparrow$} & \shortstack{Stretch\\$\downarrow$} & \shortstack{Concept\\$\uparrow$} & \shortstack{Reads as\\letter $\uparrow$} & \shortstack{Form\\weight $\to 1$} \\
\midrule
\multicolumn{10}{l}{\emph{Full task}} \\
DT                        & $7.23$ & $6.28$ & $2.67$ & $\mathbf{0.6\%}$ & $0.950$ & $9.05$ & $18.23$ & $\mathbf{51\%}$ & $0.96$ \\
Astra                     & $9.26$ & $\mathbf{12.40}$ & $\mathbf{0.25}$ & $49.1\%$ & $\mathbf{0.976}$ & $\mathbf{1.47}$ & $19.08$ & $32\%$ & $0.81$ \\
Ours                      & $\mathbf{6.11}$ & $9.24$ & $0.84$ & $1.1\%$ & $0.966$ & $3.32$ & $\mathbf{19.54}$ & $48\%$ & $\mathbf{1.01}$ \\
\midrule
\multicolumn{10}{l}{\emph{Frozen shape}} \\
AniClipart                & $9.14$ & $5.22$ & $1.58$ & $\mathbf{0.3\%}$ & $0.981$ & $1.24$ & $18.67$ & $56\%$ & $0.97$ \\
Astra                     & $\mathbf{2.49}$ & $2.03$ & $\mathbf{0.55}$ & $13.1\%$ & $\mathbf{0.998}$ & $\mathbf{1.11}$ & $18.35$ & $\mathbf{67\%}$ & $0.97$ \\
Ours                      & $7.72$ & $\mathbf{10.83}$ & $0.92$ & $1.6\%$ & $0.966$ & $2.03$ & $\mathbf{18.86}$ & $57\%$ & $0.97$ \\
\bottomrule
\end{tabular*}
\end{table}

